Improved Deterministic $(\Delta+1)$-Coloring in Low-Space MPC

We present a deterministic $O(\log \log \log n)$-round low-space Massively Parallel Computation (MPC) algorithm for the classical problem of $(\Delta+1)$-coloring on $n$-vertex graphs. In this model, every machine has a sublinear local memory of size $n^{\phi}$ for any arbitrary constant $\phi \in (0,1)$. Our algorithm works under the relaxed setting where each machine is allowed to perform exponential (in $n^{\phi}$) local computation, while respecting the $n^{\phi}$ space and bandwidth limitations. Our key technical contribution is a novel derandomization of the ingenious $(\Delta+1)$-coloring LOCAL algorithm by Chang-Li-Pettie (STOC 2018, SIAM J. Comput. 2020). The Chang-Li-Pettie algorithm runs in $T_{local}=poly(\log\log n)$ rounds, which sets the state-of-the-art randomized round complexity for the problem in the local model. Our derandomization employs a combination of tools, most notably pseudorandom generators (PRG) and bounded-independence hash functions. The achieved round complexity of $O(\log\log\log n)$ rounds matches the bound of $\log(T_{local})$, which currently serves an upper bound barrier for all known randomized algorithms for locally-checkable problems in this model. Furthermore, no deterministic sublogarithmic low-space MPC algorithms for the $(\Delta+1)$-coloring problem were previously known.

==> derand-CLP.tex <==
\section{Improved Coloring via Derandomization of CLP}\label{sec:derand}
In this section, we show a deterministic coloring algorithm that runs in $O(\log\log\log n)$ rounds, by derandomizing the CLP algorithm of \cite{chang2020distributed}. In contrast to the algorithm presented in the previous section, the local computation time (at each machine) might be exponential but the space bounds are kept to $n^{\delta}$. We show

\begin{theorem}\label{thm:col-improved}
There is a deterministic algorithm with heavy local computation for computing $(\Delta+1)$ list coloring in $O(\log\log\log n)$ rounds in the MPC model with local space $n^{\delta}$. 
\end{theorem}

Throughout, we assume that $\Delta \in [\log^c n, n^{\delta/c}]$ for some constant $c$. We start by computing $\Delta^{2t}$ coloring, for some constant $t$, to assign each vertex an identifier of $O(\log \Delta)$ bits.
Our goal would be to derandomize a $t=O(1)$ round local algorithm and thus the identifiers assigned are unique in the eyes of such an algorithm, and we can therefore treat these colors as IDs with $O(\log \Delta)$ bits. 

The main part of our algorithm colors subset of the vertices in $O(\log\log\log n)$ deterministic rounds, such that the degree of the remaining uncolored subgraph is at most poly-logarithmic. Once the degrees are that small, we can complete the coloring in $O(\log\log\log n)$ rounds, by derandomizing the classic local algorithm for $(deg+1)$ coloring. 


\subsection{Pseudo Random Generators}\label{sec:PRG}
\input{PRG.tex}



%Let $n^{\delta}$ be the local space of each machine. We claim the following.



\subsection{High Level Description of CLP}\label{sec:CLP-high}

\paragraph{High-level Description of the CLP Alg. in the \local\ Model.}
In the description below, we focus on the main randomized part of the CLP algorithm \cite{harris2016distributed}, and start by providing key definitions and ideas from \cite{harris2016distributed}. %We start by describing the main part of Harris-Schneider-Su algorithm \cite{harris2016distributed}. 
%Schneider and Wattenhofer showed an $O(\log^* n)$-round algorithm when the palette size is $(1+\epsilon)\Delta$ for constant $\epsilon \in [0,1]$. 

Harris-Schneider-Su algorithm is based on partitioning the graph into an $\epsilon$-sparse subgraph and a collection of vertex-disjoint $\epsilon$-dense components, for a given input parameter $\epsilon$. 
Since the CLP algorithm extends this partitioning, we next formally provide the basic definitions from \cite{harris2016distributed}.
For an $\epsilon \in (0,1)$, an edge $e=(u,v)$ is an $\epsilon$-friend if $|N(u) \cap N(v)|\geq (1-\epsilon)\cdot \Delta$. The endpoints of an $\epsilon$-friend edge are $\epsilon$-friends.
A vertex $v$ is $\epsilon$-dense if $v$ has at least $(1-\epsilon)\Delta$ $\epsilon$-friends, otherwise it is $\epsilon$-sparse. %When $\Delta=O(\sqrt{n})$, each vertex can collect the neighbors of its neighbors in $O(1)$ rounds, compute its $\epsilon$-friends, and decide if it is an $\epsilon$-dense or $\epsilon$-sparse. 
A key structure that arises from the definition of $\epsilon$ dense vertices is that of $\epsilon$-\emph{almost clique} which is a connected component of the subgraph induced by the $\epsilon$-dense vertices and $\epsilon$-friend edges. 
The dense components, $\epsilon$-\emph{almost} cliques, have some nice properties: each component $C$ has at most $(1+\epsilon)\Delta$ many vertices, each vertex $v \in C$ has $O(\epsilon \Delta)$ neighbors outside $C$ (called \emph{external} neighbors) and $O(\epsilon\Delta)$ vertices in $C$ which are not its neighbors. In addition, $C$ has weak diameter at most $2$. Coloring the dense vertices consists of $O(\log_{1/\epsilon} \Delta)$ phases. 
The efficient coloring of dense regions is made possible by generating a random proper coloring inside each clique so that each vertex has a small probability of receiving the same color as one of its external neighbors. 
To do that, in each cluster a random permutation is computed and each vertex selects a tentative color from its palette excluding the colors selected by
lower rank vertices. Since each component has weak diameter at most $2$, this process is implemented in $2$ rounds of the \local\ model. The remaining \emph{sparse} subgraph is colored using a Schneider-Wattenhofer style algorithm \cite{schneider2010new} within $O(\log(1/\epsilon))$ rounds. 


In Chang-Li-Pettie algorithm the vertices are partitioned into $\ell=\lceil \log\log \Delta \rceil$ layers in decreasing level of density. This hierarchical partitioning is based on a sequence of $\ell$ sparsity thresholds $\epsilon_1,\ldots,\epsilon_\ell$ where $\epsilon_i=\sqrt{\epsilon_{i-1}}$. Roughly speaking, level $i$ consists of the vertices which are $\epsilon_i$-dense but $\epsilon_{i-1}$-sparse.
Instead of coloring the vertices layer by layer, the algorithm partitions the vertices in level $i$ into large and small components and partitions the layers into $O(\log^* \Delta)$ strata, vertices in the same stratum would be colored simultaneously.  The algorithm colors vertices in $O(\log^* \Delta)$ phases, giving priority to vertices in small components. The procedures that color the dense vertices are of the same flavor as those of Harris-Schneider-Su. The key benefit in having the hierarchical structure is that the dense-coloring procedure is applied for $O(1)$ many phases on each stratum, rather than applying it for $O(\log_{1/\epsilon}\Delta)$ phases as in \cite{harris2016distributed}. 

\subsection{Initial Slack Generation}\label{sec:slack}
The CLP algorithm starts by applying a $O(1)$-round randomized procedure $\OneShotColoring$ which translates the sparsity in vertices neighborhoods into a slack in the number of colors. In this procedure, each uncolored node participates with probability $p$, and each participating vertex $v$ randomly selects a color $c(v)$ from its palette $\Pal(v)$. This color is selected for $v$ only if none of its neighbors picked that color. 
We first show that the $\OneShotColoring$ satisfies the desired slackness properties even when the random decisions made by the vertices are not fully independent, but rather almost $O(\log n)$-wise independent. 


\begin{theorem}\label{thm:one-shot-almost}[Partial Derandomization of Lemma 2.5 from \cite{chang2020distributed}]
%Let $\mathcal{H}$ be a family of $O(\log n)$-wise independent hash functions from Fact \ref{cor:hashschedule}. 
There is a $O(1)$-time algorithm (in the local model) that given a shared random seed of $O(\log n)$ bits (and no other source of randomness) colors a subset of the vertices $V$, such that the following are true for each $v$ with $deg(v)\geq (5/6)\Delta$:
\begin{itemize}
\item{(P1)} With probability $1-1/n^c$, the number of uncolored neighbors of $v$ is at least $\Delta/2$.
\item{(P2)} With probability $1-1/n^c$, $v$ has at least $\Omega(\epsilon^2 \Delta)$ excess colors, where $\epsilon$ is the highest value such that $v$ is $\epsilon$-sparse for $\epsilon\geq 1/\Delta^{1/10}$.
\end{itemize}
\end{theorem}
We provide the proof of Theorem \ref{thm:one-shot-almost} in Appendix \ref{app:one-shot-almost}. Next, we show that the randomized algorithm of Theorem \ref{thm:one-shot-almost} can be derandomized within $O(1)$ number of rounds. 

Next, we show that the algorithm of Theorem \ref{thm:one-shot-almost} can be made deterministic by using the standard method of conditional expectation.
\begin{lemma}\label{lem:one-shot-derand}
The algorithm of Theorem \ref{thm:one-shot-almost} can be fully derandomized within $O(1)$ deterministic rounds, where all vertices $v$ with $deg(v)\geq (5/6)\Delta$ satisfy properties (P1) and (P2). 
\end{lemma}
\begin{proof}
Let $K=\ell\log n$ be seed length used to implement the algorithm of Theorem \ref{thm:one-shot-almost}. The algorithm applies $O(\ell)$ steps where in each step a chunk of $\lfloor \log n \rfloor$ bits in the seed are computed via the method of conditional expectation. 

Throughout, we assume that we have at least $n$ machines, where machine $M_u$ stores the $2$-hop ball of vertex $u$. 
For every possible $\lfloor \log n \rfloor$-bit vector $Q$ we have a designated machine $M_Q$ whose role in phase $i$ is to evaluate the progress given that the assignment to the $i^{th}$ chunk in the seed is $Q$. We now explain the $i^{th}$ phase and let $Z' \in \{0,1\}^{(i-1)\lfloor \log n \rfloor}$ be the prefix of the seed already computed in phase $1,\ldots, i-1$.

For a given complete seed $Z \in \{0,1\}^K$, a vertex $u$ is \emph{happy} if both properties (P1) and (P2) hold when picking the random colors based on $h_Z$ where $h_Z$ is the function chosen from $\mathcal{H}$ given $Z$. 
For every $Q \in \{0,1\}^{\lfloor \log n \rfloor}$, each machine $M_u$ computes the probability that $u$ is happy, when fixing the prefix of the seed to $Z' \circ Q$. Since the happiness of a vertex depends only on the choices of itself and its immediate neighbors, $M_u$ can indeed compute this probability. 
This information is then sent to machine $M_Q$ using the standard routing technique. Within $O(1/\delta)$ rounds, each machine $M_Q$ computes the expected number of happy vertices conditioned on the prefix $Z' \circ Q$. The elected $i^{th}$ chunk $Q^*$ is the one the maximizes the conditional expectation. After $\ell$ such phases the selected seed $Z^*$. Since the expected number of happy vertices under random seed is $n$, by the method of conditional expectation, the number of happy vertices under $Z^*$ is $n$ as well. 
%We start by describing the first phase for determining the first $\lfloor \log n\rfloor$. For each assignment $Z_1 \in \{0,1\}^{\lfloor \log n\rfloor}$, machine $M_u$ computes the fraction of seeds with prefix $Z_1$ in which $u$ is \emph{happy}. For each such $Z_1$, the algorithm assigns a designated machine $M_{Z_1}$ that computes the expected number of happy vertices under $Z_1$. The elected prefix is the one that maximizes that value. All this operations can be done in $O(1)$ rounds. The process continues where in the $i^{th}$ phase, we compute the conditional expectation of the number of happy nodes under the $i^{th}$ chunk $Z_i \in \{0,1\}^{\lfloor \log n\rfloor}$ conditioned on the $(i-1)$ chuncks computed in previous phases.
\end{proof}





\subsection{Dense Coloring}\label{sec:dense-col} 
The dense coloring procedures of \cite{chang2020distributed} are based on collecting the vertices of each almost-clique $C$ to a leader vertex $u \in C$ which permutes the vertices and color them sequentially. While it not clear how to derandomize it using a small logarithmic seed in polynomial time, it is possible to derandomize in local exponential time, locally at each machine. 


\subsubsection{Coloring Small and Medium Blocks}\label{sec:small-med-col}





\subsection{Dense Coloring with No Slack}



%\begin{definition}
%An ordered partitioning of the block set $\mathcal{B}$ into $\{L_1,\ldots, L_k\}$ \emph{satisfies} property $\pi$ if 
%for every $j \in \{1,\ldots, k\}$ and every block $B \in L_j$, it holds that $B$ satisfies property $\pi$ in the subgraph induced on the union of blocks $\bigcup_{j' \leq j} L_{j'}$.
%\end{definition}
%
%\begin{definition}[Block-monotonic property]
%A property $\pi$ defined for a graph $G$ and a partial coloring of it is said to be \emph{block-monotonic} if given the all vertices in block $B$ satisfy $\pi$, they also satisfy it in any subgraph $G'$ of $G$ that contains $B$, where the vertices in $G'$ maintain their color. 
%\end{definition}
%
%
%
%
%\begin{theorem}\label{thm:det-property}
%Let $\mathcal{B}=\{S_1,\ldots, S_g\}$ be a collection of blocks. Suppose there is a $O(1)$-time randomized algorithm that colors a subset of the vertices in $\bigcup S_j$ such that w.h.p. the one-hop ball of each $S_j$ satisfies some desired property $\pi$. Then, there is a $O(1)$ time deterministic algorithm that computes an ordered subsets of blocks $L_1, \ldots, L_k$ for $k=O(1)$ that satisfies property $\pi$. 
%\end{theorem}
%
%We start by providing the key auxiliary lemma which uses the PRG machinery to satisfy the requirement for 
%\begin{lemma}\label{lem:det-property-aux}
%Let $\mathcal{B}=\{S_1,\ldots, S_g\}$ be a collection of blocks. Suppose there is a $O(1)$-time local randomized algorithm $\cA$ that colors a subset of the vertices in $\bigcup S_j$ such that w.h.p. the one-hop ball of each $S_j$ satisfies some desired property $\pi$. In addition, the local computation performed by each vertex in algorithm $\cA$ is polynomial. Then, there is a $O(1)$ time deterministic algorithm that computes a partial coloring to all vertices in the blocks of $\mathcal{B}$ such that at least $1-1/n^{\alpha}$-fraction of the blocks satisfies the property $\pi$ under that coloring. 
%\end{lemma}
%\begin{proof}
%The $O(1)$-time randomized algorithm satisfies the desired property for all vertices in the blocks of $\mathcal{B}$ w.h.p. In our derandomization scheme, when using the PRG, we obtain an almost-high probability guarantee of $p=1-1/n^{\alpha}$ for some constant $\alpha \in (0,1)$. We call a block $B \in \mathcal{B}'$ \emph{happy} if all its vertices satisfy property $\pi$. Our goal is to provide a partial coloring to the vertices in $\mathcal{B}$ such that at least $(1-1/n^{\alpha})$ fraction of the blocks are happy. 
%
%For each block $B$, we allocate a machine $M_B$ that stores the $2t$-radius ball of the vertices of $B$ where $t$ is the running time of the randomized algorithm. By proposition \ref{prop:perfect-PRG}, there exists an $(\poly(\Delta),1/n^{\alpha})$ pseudorandom generator with seed length of $d=\log n/\alpha$ which can fool any $\poly(\Delta)$-time computation with error of $1/n^{\alpha}$. This seed can be computed by Lemma \ref{lem:prg-alg} using space of $2^{O(d)}=O(n^{\delta})$ for a sufficiently small constant $\alpha$, which fits the local space of the machines.  
%
%It is convenient to view the local randomized algorithm $\cA$ as an algorithm runs by a leader of each block. Each vertex uses $O(\log \Delta)$ many random bits and the machine storing a vertex also holds it random coins (so that the randomized decisions made by a vertex are consistent across all machines that store it). 
%Since the local computation of algorithm $\cA$ is polynomial in time, hence $\poly(\Delta)$ time in our context, using the above explanation that is a seed of length $o(\log n/\delta)$ such that $\epsilon$-fools the local computation of each leader in algorithm $\cA$ for $\epsilon = 1/n^{\alpha}$. Since the randomized local computation algorithm at each leader succeeds in satisfying $\pi$ w.h.p. for all vertices in the block, using a pseudo-random coins obtained by applying the PRG on a random seed with $d$ bits fails with probability at most $2/n^{1/\alpha}$. 
%Therefore, in expectation over $Z \in \{0,1\}^d$, there are at least $1-1/n^{\alpha}$ fraction of happy blocks in $\mathcal{B}'$. 
%
%Since we use $O(\log\Delta)$-bit identifiers to the vertices, for a given fixed seed $Z \in \{0,1\}^d$, the coloring decision computed for a given vertex by distinct machines that hold that vertex are consistent. Our goal is then to compute a seed $Z^* \in \{0,1\}^d$ that achieves the desired expected value of happy vertices. To do that, the algorithm assigns a machine $M_Z$ for each possible seed $Z \in \{0,1\}^d$. Each machine $M_B$ then sends to $M_Z$ a score of $1$ if $B$ is happy under $Z$, and a score of $0$, otherwise. The selected seed $Z^*$ is the seed that got the maximal number of happy nodes. The lemma follows.
%\end{proof}
%
%\begin{theorem}\label{thm:det-property}
%Let $\mathcal{B}=\{S_1,\ldots, S_g\}$ be a collection of blocks. Suppose there is a $O(1)$-time randomized algorithm that colors a subset of the vertices in $\bigcup S_j$ such that w.h.p. the one-hop ball of each $S_j$ satisfies some desired property $\pi$. Then, there is a $O(1)$ time deterministic algorithm that computes an ordered subsets of blocks $L_1, \ldots, L_k$ for $k=O(1)$ that satisfies property $\pi$. 
%\end{theorem}

At first glance it might appear that Theorem \ref{thm:det-property} can be obtained by having $O(1/\alpha)$ repetitions of the algorithm of Lemma \ref{lem:det-property-aux}. This is because Lemma \ref{lem:det-property-aux}
covers a large fraction of the blocks, and thus within $O(1/\alpha)$  applications all blocks should be covered. This solution, however, fails for the following reason.  The colors assigned to the vertices for the unhappy blocks in a given application of Lemma \ref{lem:det-property-aux} might ruin their chances to ever satisfy $\pi$. Therefore, in principle, colors assigned to unhappy blocks should not be adopted. The problem with that is the dependency between blocks: happy blocks might become unhappy upon the cancellation of the coloring to the unhappy blocks. Theorem \ref{thm:det-property} handles this situation by using a relaxed notion of \emph{satisfying a property}, which we found to be sufficient in our context. 


\begin{lemma}\label{det-dense-step}
Let $\mathcal{B}=\{B_1,\ldots, B_\ell\}$ be a collection of blocks and let $\mathcal{B}' \subseteq \mathcal{B}$ be a subset of blocks that satisfies the $i^{th}$ invariant w.r.t the current coloring of all blocks in $\mathcal{B}$.
Then, there is a $O(1)$-round deterministic procedure for coloring a subset of vertices in $\mathcal{B}'$, such that at least $(1-1/n^{\alpha})$-fraction of the blocks satisfies the $(i+1)^{th}$ invariant, for some constant $\alpha \in (0,1)$.
\end{lemma}
\begin{proof}
The randomized procedure $\DenseColoringStep$ satisfies the desired property with high probability for $\Delta> \log^c n$.  In our derandomization scheme, when using the PRG, we obtain an almost-high probability guarantee of $p=1-1/n^{\alpha}$ for some constant $\alpha \in (0,1)$. We call a block $B \in \mathcal{B}'$ \emph{happy} if it satisfies the $(i+1)^{th}$ invariant. For each block $B$, we allocate a machine $M_B$ that stores all the edges and vertices of the block $B$.

Specifically, by proposition \ref{prop:perfect-PRG}, there exists an $(\poly(\Delta),1/n^{\alpha})$ pseudorandom generator with seed length of $d=\log n/\alpha$ which can fool any $\poly(\Delta)$-time computation with error of $1/n^{\alpha}$. This seed can be computed by Lemma \ref{lem:prg-alg} using space of $2^{O(d)}=O( n^{\delta})$ for a sufficiently small constant $\alpha$, which fits the local space of the machines.  Since the local computation of Procedure $\DenseColoringStep$ applied by the block leader is polynomial, the machines can compute a seed that fools all these algorithms up to small error of $1/n^{\alpha}$. The fully randomized $\poly(\Delta)$-time algorithm $T$ applied by each block' leader guarantees that w.h.p. all blocks are happy. Using a pseudo random string obtained from a $d$-length random seed $Z$ provides a success guarantee of $1-1/n^{\alpha}$. Therefore, in expectation over $Z \in \{0,1\}^d$, there are at least $1-1/n^{\alpha}$ fraction of happy blocks in $\mathcal{B}'$. 

Since we use $O(\log\Delta)$-bit identifiers to the vertices, for a given fixed seed $Z \in \{0,1\}^d$, the coloring decision computed for a given vertex by distinct machines that hold that vertex are consistent. Our goal is then to compute a seed $Z^* \in \{0,1\}^d$ that achieves the desired expected value of happy vertices. To do that, the algorithm assigns a machine $M_Z$ for each possible seed $Z \in \{0,1\}^d$. Each machine $M_B$ then sends to $M_Z$ a score of $1$ if $B$ is happy under $Z$, and a score of $0$, otherwise. The selected seed $Z^*$ is the seed that got the maximal number of happy nodes. The lemma follows.
\end{proof}


%\begin{observation}\label{obs:monotonic}
%Consider a graph with partial coloring $\pi$ where a block $B$ satisfies invariant $k$ with respect to $\pi$. Then in any coloring $\pi'$ that extends $\pi$, the block $B$ satisfies the invariant $k$ under a coloring $\phi''$ that agrees with $\pi'$ on all vertices not in $B$, and agrees with $\p$ with all vertices in $B$. 
%\end{observation}

We start by providing the key auxiliary lemma which uses the PRG machinery to satisfy the invariant for most of the blocks.



\begin{lemma}\label{lem:det-property-aux}
Let $\mathcal{B}=\{S_1,\ldots, S_g\}$ be a collection of blocks. Suppose there is a $O(1)$-time local randomized algorithm $\cA$ that colors a subset of the vertices in $\bigcup S_j$ such that w.h.p. the one-hop ball of each $S_j$ satisfies some desired property $\pi$. In addition, the local computation performed by each vertex in algorithm $\cA$ is polynomial. Then, there is a $O(1)$ time deterministic algorithm that computes a partial coloring to all vertices in the blocks of $\mathcal{B}$ such that at least $1-1/n^{\alpha}$-fraction of the blocks satisfies the property $\pi$ under that coloring. 
\end{lemma}
\begin{proof}
The $O(1)$-time randomized algorithm satisfies the desired property for all vertices in the blocks of $\mathcal{B}$ w.h.p. In our derandomization scheme, when using the PRG, we obtain an almost-high probability guarantee of $p=1-1/n^{\alpha}$ for some constant $\alpha \in (0,1)$. We call a block $B \in \mathcal{B}'$ \emph{happy} if all its vertices satisfy property $\pi$. Our goal is to provide a partial coloring to the vertices in $\mathcal{B}$ such that at least $(1-1/n^{\alpha})$ fraction of the blocks are happy. 

For each block $B$, we allocate a machine $M_B$ that stores the $2t$-radius ball of the vertices of $B$ where $t$ is the running time of the randomized algorithm. By proposition \ref{prop:perfect-PRG}, there exists an $(\poly(\Delta),1/n^{\alpha})$ pseudorandom generator with seed length of $d=\log n/\alpha$ which can fool any $\poly(\Delta)$-time computation with error of $1/n^{\alpha}$. This seed can be computed by Lemma \ref{lem:prg-alg} using space of $2^{O(d)}=O(n^{\delta})$ for a sufficiently small constant $\alpha$, which fits the local space of the machines.  

It is convenient to view the local randomized algorithm $\cA$ as an algorithm runs by a leader of each block. Each vertex uses $O(\log \Delta)$ many random bits and the machine storing a vertex also holds it random coins (so that the randomized decisions made by a vertex are consistent across all machines that store it). 
Since the local computation of algorithm $\cA$ is polynomial in time, hence $\poly(\Delta)$ time in our context, using the above explanation that is a seed of length $o(\log n/\delta)$ such that $\epsilon$-fools the local computation of each leader in algorithm $\cA$ for $\epsilon = 1/n^{\alpha}$. Since the randomized local computation algorithm at each leader succeeds in satisfying $\pi$ w.h.p. for all vertices in the block, using a pseudo-random coins obtained by applying the PRG on a random seed with $d$ bits fails with probability at most $2/n^{1/\alpha}$. 
Therefore, in expectation over $Z \in \{0,1\}^d$, there are at least $1-1/n^{\alpha}$ fraction of happy blocks in $\mathcal{B}'$. 

Since we use $O(\log\Delta)$-bit identifiers to the vertices, for a given fixed seed $Z \in \{0,1\}^d$, the coloring decision computed for a given vertex by distinct machines that hold that vertex are consistent. Our goal is then to compute a seed $Z^* \in \{0,1\}^d$ that achieves the desired expected value of happy vertices. To do that, the algorithm assigns a machine $M_Z$ for each possible seed $Z \in \{0,1\}^d$. Each machine $M_B$ then sends to $M_Z$ a score of $1$ if $B$ is happy under $Z$, and a score of $0$, otherwise. The selected seed $Z^*$ is the seed that got the maximal number of happy nodes. The lemma follows.
\end{proof}


\begin{theorem}
Assume there exists a $O(1)$-round randomized algorithm that is made of $\beta$ phases such that given that all vertices satisfy invariant $i$ at the beginning of phase $i$ computes an extension of the coloring such that w.h.p. all vertices satisfy invariant $i+1$. Then there exists a $O(1)$ round algorithm that outputs a partial coloring, and an ordered partitioning $L_1,\ldots, L_k$ for $k=O(1)$ that satisfies invariant $\beta$. 
\end{theorem}
The algorithm has $\beta=12$ phases, where at the end of these phases, we will have an ordered collection of block-subsets $L_1,\ldots, L_k$ such that each vertex $u$ in a block $B \in L_j$ has at most poly-logarithmic number of neighbors in the blocks of $\bigcup_{j' \leq j} L_{j'}$. 

\paragraph{Phase $i$.} The goal of the $i^{th}$ phase is to compute a partial coloring such that the collection of blocks \emph{satisfy} the $(i+1)^{th}$ invariant under some relaxed notion as defined next.

\begin{definition}
For every $i \in \{1,\ldots,\beta\}$, an ordered partitioning of the block set $\mathcal{B}$ into $\{L_1,\ldots, L_k\}$ \emph{satisfies} the $i^{th}$ invariant if for every $j \in \{1,\ldots, k\}$ and every block $B \in L_j$, it holds that $B$ satisfies the $i^{th}$ invariant with respect to the union of blocks $\bigcup_{j' \leq j} L_{j'}$. 
\end{definition}


The input to the $i^{th}$ phase is an ordered partitioning $L_{i,1}, \ldots, L_{i,n_i}$ that satisfies the $i^{th}$ invariant, and such that $n_i\leq (c/\alpha)^{i-1}$. The output of the phase is an ordered partitioning $L_{i+1,1}, \ldots, L_{i+1,n_{i+1}}$ that satisfies the $(i+1)^{th}$ invariant, and such that $n_{i+1}\leq (c/\alpha)^{i}$. The algorithm processes the block subsets $L_{i,1}, \ldots, L_{i,n_i}$ in a sequential manner, one by one. 
Consider the $j^{th}$ step when it considers the sub-set $L_{i,j}$. The algorithm makes $K=c/\alpha$ applications of algorithm $P$ from Lemma \ref{det-dense-step} on the blocks of $L_{i,j}$. 
For every application $\ell$, let $L_{i,j,\ell}$ be the collection of new happy blocks added in the $\ell^{th}$ application.
We will show that $K$ applications are in fact sufficient. 
Let $L'_{i,j,\ell} \subseteq L_{i,j}$ be the subset of yet unhappy blocks in $L_{i,j}$ at the beginning of the $\ell^{th}$ application.  I.e., $L'_{i,j,\ell}=L_{i,j} \setminus \bigcup_{\ell'\leq  \ell-1} L_{i,j,\ell'}$. 

Note that the blocks of $L'_{i,j,\ell}$ did not yet adapt any of the coloring of algorithm $P$ to their vertices. Therefore their block size and anti-degree are unchanged, and their external degree is not larger compared to the beginning of the $i^{th}$ phase. Therefore, all blocks in $L'_{i,j,\ell}$ satisfy the $i^{th}$ invariant w.r.t to all blocks in $\bigcup_{j' \leq j }L_{i,j'}$. 

We can then safely apply algorithm $P$ with $\mathcal{B}=\bigcup_{j' \leq j }L_{j'}$ and $\mathcal{B}'=L'_{i,j,\ell}$. Algorithm $P$ returns a subset $L_{i,j,\ell} \subseteq L'_{i,j,\ell}$ of happy blocks that satisfy invariant $(i+1)$ and $L_{i,j,\ell}$ contains at least $(1-1/n^{\alpha})$ fraction of the blocks in $L'_{i,j,\ell}$. After $K$ applications of algorithm $P$, we get the ordered partitioning of $L_{i,j}$ given by $L_{i,j,1}, \ldots, L_{i,j,K}$ that satisfy the $(i+1)^{th}$ invariant.


We now claim that resulting ordered set obtained by $n_i \cdot K$ sequential  applications of algorithm $P$, namely,
$$L_{i,1,1},\ldots, L_{i,1,K}, L_{2,1,1},\ldots, L_{2,1,K}, \ldots, L_{n_i,1,1},\ldots, L_{n_i,1,K},$$
satisfies the $(i+1)$ invariants. This completes the description of the $i^{th}$ phase. 
The $\beta=12$ invariant of the algorithm (see \cite{chang2020distributed}) states that the block size as well as the external degrees are poly-logarithmic. Since we obtain an ordered set of $K^{\beta}$ block subsets that satisfy the $\beta^{th}$ invariant, the claim holds.  



\paragraph{Coloring Layer-$2^+$ Large Blocks.}

The invariant $k$ requires bounds $U^{(k)}_{j}$, $L^{(k)}_{j}$ and $D^{(k)}_{j}$ as well as having at most $\delta^{(k)}_i \cdot \Delta$ uncolored $i$-layer neighbors for every vertex in the block. 
Observe that these invariants are block-monotone. In the randomized algorithm of \cite{chang2020distributed}, the $6^{th}$ invariant guarantees that each vertex has at most $\epsilon_i^5 \Delta$ uncolored layer-$i$ neighbors. 




\subsubsection{Coloring Layer-1 Large Blocks}\label{sec:large-col-one}
We start by considering the most challenging step of coloring the large blocks in layer-1. These nodes have no guaranteed slack in their palettes, and the ordering in which the algorithm colors these vertices plays a critical role. We present a $O(1)$-time algorithm that colors a subset of the vertices in these large blocks such that one can orient the remaining uncolored subgraph in a way that guarantees a poly-logarithmic out-degree.

\begin{theorem}\label{thm:det-coloring-large-one}
There exists a deterministic procedure that colors a subset of vertices in the collection of layer-1 large blocks $\mathcal{B}$. Letting $G'$ be the subgraph induced by the uncolored vertices in $\mathcal{B}$, then there exists an orientation $\bar{G}'$ of $G'$ such that the out-degree of $\bar{G}'$ is poly-logarithmic.
\end{theorem}

The algorithm of \cite{chang2020distributed} is based on having $\beta=12$ iterations of Procedure $\DenseColoringStep$ (version 2) until the maximum degree becomes poly-logarithmic. In each iteration $i$, there is an invariant $i$ on the cluster size expressed by upper bound $U_i$ and lower bound $L_i$, as well as an upper bound $D_i$ on the anti-degree and the external degrees. For $i=\beta$, the bounds $U_{\beta}, L_{\beta}$ and $D_{\beta}$ are all poly-logarithmic. Under these invariants, the $i^{th}$ application of $\DenseColoringStep$ provides a shrinking rate $O(\delta_i)$ where 
$$\delta_i = \frac{D_i\log(L_i/D_i)}{L_i}~.$$
For $\Delta> \log^c n$, the analysis of \cite{chang2020distributed} shows that after the $i^{th}$ application of Procedure $\DenseColoringStep$ all blocks satisfy the $(i+1)$ invariant with probability of $1-1/n^c$. Due to the sub-linear space limitation of our machines, we cannot provide such a small error. Instead, we can only guarantee the invariant to hold with probability of $1-1/n^{\alpha}$ for a sufficiently small constant $\alpha \in (0,1)$, to be set later. 
This larger error poses a great challenge for the deterministic algorithm, and in particular, we would not be able to mimic the randomized procedure (and its subsequent analysis) as in \cite{chang2020distributed}. We start by providing the basic deterministic procedure to be used in our solution. 

\begin{lemma}\label{rand-dense-step}
Let $\mathcal{B}' \subseteq \mathcal{B}$ be a subset of blocks 
such that each $B \in \mathcal{B}'$ satisfies:
\begin{itemize}
\item the $(i+1)^{th}$ neighbor-invariant w.r.t its neighbors in $\mathcal{B} \setminus \mathcal{B}'$.
\item the $i^{th}$ neighbor-invariant w.r.t its neighbors in $\mathcal{B}'$, and
\item the $i^{th}$ self-invariant.
\end{itemize}
Then, there is a $O(1)$-round randomized procedure applied only by the vertices in $\mathcal{B}$ such that w.h.p., every $B \in \mathcal{B}'$  
\begin{itemize}
\item{(i)} satisfies $(i+1)^{th}$ invariant, and 
\item{(ii)} does not violate the $(i+1)^{th}$ invariant for its neighbors in $\mathcal{B}\setminus \mathcal{B}'$. 
\end{itemize}
\end{lemma}



\begin{lemma}\label{det-dense-step}
Let $\mathcal{B}' \subseteq \mathcal{B}$ be a subset of blocks 
such that each $B \in \mathcal{B}'$ satisfies:
\begin{itemize}
\item the $(i+1)^{th}$ neighbor-invariant w.r.t its neighbors in $\mathcal{B} \setminus \mathcal{B}'$.
\item the $i^{th}$ neighbor-invariant w.r.t its neighbors in $\mathcal{B}'$, and
\item the $i^{th}$ self-invariant.
\end{itemize}
Then, there is a $O(1)$-round deterministic procedure for coloring a subset of vertices in $\mathcal{B}'$ as well as a subset $\mathcal{B}''\subseteq \mathcal{B}'$, where $|\mathcal{B}''|\geq (1-1/n^{\alpha})|\mathcal{B}'|$ such that for each $B \in \mathcal{B}''$ it holds that every $B' \in N^+(B)$  
\begin{itemize}
\item{(i)} satisfies $(i+1)^{th}$ invariant, and 
\item{(ii)} does not violate the $(i+1)^{th}$ invariant for its neighbors in $\mathcal{B}\setminus \mathcal{B}'$. 
\end{itemize}
\end{lemma}
\begin{proof}
Note that our goal is to color only blocks in $\mathcal{B}'$ and all blocks in $\mathcal{B}\setminus \mathcal{B}'$ should keep their given color. Since the neighbors of block $B \in \mathcal{B}'$ in $\mathcal{B}\setminus \mathcal{B}'$ already satisfy the $(i+1)^{th}$ neighbor-invariant, we do not need any recoloring of the vertices in $\mathcal{B}\setminus \mathcal{B}'$. Therefore it is only required for $B$ to satisfy the $(i+1)^{th}$ self-invariant and the 
$(i+1)^{th}$ neighbor-invariant of $B$ w.r.t its neighbors in $\mathcal{B}'$, as well as, to maintain the $(i+1)^{th}$ neighbor-invariant of its neighbors in $\mathcal{B} \setminus \mathcal{B}'$. 

By Lemma \ref{rand-dense-step}, the randomized procedure $\DenseColoringStep$ satisfies the desired property with high probability for $\Delta> \log^c n$.  In our derandomization scheme, when using the PRG, we obtain an almost-high probability guarantee of $p=1-1/n^{\alpha}$ for some constant $\alpha \in (0,1)$. We call a block $B \in \mathcal{B}'$ \emph{happy} if it satisfies the $(i+1)^{th}$ invariant and all its block neighbors in $\mathcal{B}'$ also satisfy the $(i+1)^{th}$ invariant. For each block $B$, we allocate a machine $M_B$ that stores the $2$-hop neighboring blocks of $B$. The block $B$ is \emph{happy} if $B$ and all its block-neighbors satisfy properties (i) and (ii).

Specifically, by proposition \ref{prop:perfect-PRG}, there exists an $(\poly(\Delta),1/n^{\alpha})$ pseudorandom generator with seed length of $d=\log n/\alpha$ which can fool any $\poly(\Delta)$-time computation with error of $1/n^{\alpha}$. This seed can be computed by Lemma \ref{lem:prg-alg} using space of $2^{O(d)}=O( n^{\delta})$ for a sufficiently small constant $\alpha$, which fits the local space of the machines.  Since the local computation of Procedure $\DenseColoringStep$ applied by the block leader is polynomial, the machines can compute a seed that fools all these algorithms up to small error of $1/n^{\alpha}$. The fully randomized $\poly(\Delta)$-time algorithm $T$ applied by each block' leader guarantees that w.h.p. all blocks are happy. Using a pseudo random string obtained from a $d$-length random seed $Z$ provides a success guarantee of $1-1/n^{\alpha}$. Therefore, in expectation over $Z \in \{0,1\}^d$, there are at least $1-1/n^{\alpha}$ fraction of happy blocks in $\mathcal{B}'$. 

Since we use $O(\log\Delta)$-bit identifiers to the vertices, for a given fixed seed $Z \in \{0,1\}^d$, the coloring decision computed for a given vertex by distinct machines that hold that vertex are consistent. Our goal is then to compute a seed $Z^* \in \{0,1\}^d$ that achieves the desired expected value of happy vertices. To do that, the algorithm assigns a machine $M_Z$ for each possible seed $Z \in \{0,1\}^d$. Each machine $M_B$ then sends to $M_Z$ a score of $1$ if $B$ is happy under $Z$, and a score of $0$, otherwise. The selected seed $Z^*$ is the seed that got the maximal number of happy nodes. The lemma follows.
\end{proof}


We now provide a deterministic algorithm that is based on $(c/\alpha)^\beta$  applications of the deterministic procedure $P$ of Lemma \ref{det-dense-step} for a sufficiently large constant $c$. The algorithm has $\beta=12$ phases, where at the end of these phases, we will have an ordered collection of block-subsets $L_1,\ldots, L_k$ such that each vertex $u$ in a block $B \in L_j$ has at most poly-logarithmic number of neighbors in the blocks of $\bigcup_{j' \leq j} L_{j'}$. 

\paragraph{Phase $i$.} The goal of the $i^{th}$ phase is to compute a partial coloring such that the collection of blocks \emph{satisfy} the $(i+1)^{th}$ invariant under some relaxed notion as defined next.

\begin{definition}
For every $i \in \{1,\ldots,\beta\}$, an ordered partitioning of the block set $\mathcal{B}$ into $\{L_1,\ldots, L_k\}$ \emph{satisfies} the $i^{th}$ invariant if for every $j \in \{1,\ldots, k\}$ and every block $B \in L_j$, it holds that $B$ satisfies the $i^{th}$ invariant with respect to the union of blocks $\bigcup_{j' \leq j} L_{j'}$. 
\end{definition}


The input to the $i^{th}$ phase is an ordered partitioning $L_{i,1}, \ldots, L_{i,n_i}$ that satisfies the $i^{th}$ invariant, and such that $n_i\leq (c/\alpha)^{i-1}$. The output of the phase is an ordered partitioning $L_{i+1,1}, \ldots, L_{i+1,n_{i+1}}$ that satisfies the $(i+1)^{th}$ invariant, and such that $n_{i+1}\leq (c/\alpha)^{i}$. The algorithm processes the block subsets $L_{i,1}, \ldots, L_{i,n_i}$ in a sequential manner, one by one. 
Consider the $j^{th}$ step when it considers the sub-set $L_{i,j}$. The algorithm will make $K=c/\alpha$ applications of algorithm $P$ from Lemma \ref{det-dense-step} on the blocks of $L_{i,j}$. 
For every application $\ell$, let $L_{i,j,\ell}$ be the collection of new happy blocks added in the $\ell^{th}$ application.
We will show that $K$ applications are in fact sufficient. 
Let $L'_{i,j,\ell} \subseteq L_{i,j}$ be the subset of yet unhappy blocks in $L_{i,j}$ at the beginning of the $\ell^{th}$ application.  I.e., $L'_{i,j,\ell}=L_{i,j} \setminus \bigcup_{\ell'\leq  \ell-1} L_{i,j,\ell'}$. 

Note that the blocks of $L'_{i,j,\ell}$ did not yet adapt any of the coloring of algorithm $P$ to their vertices. Therefore their block size and anti-degree are unchanged, and their external degree is not larger compared to the beginning of the $i^{th}$ phase. Therefore, all blocks in $L'_{i,j,\ell}$ satisfy the $i^{th}$ invariant w.r.t to all blocks in $\bigcup_{j' \leq j }L_{i,j'}$. 

We can then safely apply algorithm $P$ with $\mathcal{B}=\bigcup_{j' \leq j }L_{j'}$ and $\mathcal{B}'=L'_{i,j,\ell}$. Algorithm $P$ returns a subset $L_{i,j,\ell} \subseteq L'_{i,j,\ell}$ of happy blocks that satisfy invariant $(i+1)$ and $L_{i,j,\ell}$ contains at least $(1-1/n^{\alpha})$ fraction of the blocks in $L'_{i,j,\ell}$. After $K$ applications of algorithm $P$, we get the ordered partitioning of $L_{i,j}$ given by $L_{i,j,1}, \ldots, L_{i,j,K}$ that satisfy the $(i+1)^{th}$ invariant.


We now claim that resulting ordered set obtained by $n_i \cdot K$ sequential  applications of algorithm $P$, namely,
$$L_{i,1,1},\ldots, L_{i,1,K}, L_{2,1,1},\ldots, L_{2,1,K}, \ldots, L_{n_i,1,1},\ldots, L_{n_i,1,K},$$
satisfies the $(i+1)$ invariants. This completes the description of the $i^{th}$ phase. 
The $\beta=12$ invariant of the algorithm (see \cite{chang2020distributed}) states that the block size as well as the external degrees are poly-logarithmic. Since we obtain an ordered set of $K^{\beta}$ block subsets that satisfy the $\beta^{th}$ invariant, the claim holds.  












\subsection{Sparse Coloring}\label{sec:sparse}




\subsection{Low-Deg Coloring}\label{sec:low-deg}
For this low-degree case, we can obtain an $O(\log\log\log n)$-round solution by
derandomizing a $(deg+1)$-local algorithm. 

\begin{lemma}\label{lem:low-deg}
For any $n$-vertex graph $G$ with maximum degree $\Delta=\poly\log$, there exists an $O(\log\log\log n)$-deterministic algorithm for computing $(deg+1)$ list coloring. 
\end{lemma}
\begin{proof}


\end{proof}

\subsection{High-Deg Coloring}\label{sec:low-deg}
In this section we consider the case where $\Delta=n^{\omega(\delta)}$. In order to apply our main algorithm, we first employ a vertex partitioning to reduce the degree. 

%\begin{lemma}\label{lem:high-deg}
%
%\end{lemma}
%\begin{proof}
%
%
%\end{proof}





==> shorter.tex <==

\paragraph{Coloring Layer-$2^+$ Large Blocks.}


Let $\mathcal{B}$ be a collection of all large blocks in layers $\{2,\ldots, \ell\}$. 
The property $\pi$ bounds the number of uncolored layer-$i$ neighbors by $\epsilon_i^5 \Delta$ for every vertex $v$ in the blocks of $\mathcal{B}$. Thus, this property only depends on the $1$-hop each block. 

\begin{lemma}[Implicit in \cite{chang2020distributed}]\label{lem:rand-dense-large-twoplus}
There exists a $O(1)$-round randomized algorithm that partially colors blocks $\mathcal{B}$ such that w.h.p. 
each vertex $v \in B$ for every $B \in \mathcal{B}$ has at most $\epsilon_i^5 \cdot \Delta$ uncolored layer-$i$ neighbors for every $i \in \{2,\ldots, \ell\}$. 
\end{lemma}


By applying Theorem \ref{thm:det-property} with the algorithm of Lemma \ref{lem:rand-dense-large-one} and letting $\pi$ be the required bound on the number uncolored $i$-layer neighbors for each vertex, we get:

\begin{corollary}
There exists a deterministic algorithm that computes an ordered partitioning of the large blocks in layers $[2,\ell]$ given by $L_1,\ldots, L_k$ such that $k=O(1)$, and each vertex $v \in B$ for $B \in L_j$ has at most $O(\epsilon_i^5 \Delta)$ uncolored layer-$i$ neighbors in the blocks of $L_1,\ldots, L_j$. 
\end{corollary}



\begin{corollary}
There exists a $O(\log^ \Delta)$-round deterministic algorithm for coloring all large blocks in layers $\{2,\ldots, \ell\}$.
\end{corollary}


\paragraph{Coloring Layer-$1$ Large Blocks.}

Let $\mathcal{B}$ be a collection of layer-$1$ large blocks. The property $\pi$ in our context is $\deg_U(v)\leq \log^c n$ for some constant $c$ where $\deg_U(v)$ is the uncolored degree of vertex $v$. 

\begin{lemma}[Implicit in \cite{chang2020distributed}]\label{lem:rand-dense-large-one}
There exists a $O(1)$-round randomized algorithm that partially colors the layer-1 large blocks $\mathcal{B}$ such that w.h.p. the uncolored degree of each vertex in these blocks is poly-logarithmic.
\end{lemma}

By applying Theorem \ref{thm:det-property} with the algorithm of Lemma \ref{lem:rand-dense-large-one} and letting $\pi$ be the requirement of having an uncolored poly-logarithmic degree for each vertex, we have:

\begin{corollary}
There exists a deterministic algorithm for coloring the layer-1 large blocks in $O(\log\log\log n)$ rounds.
\end{corollary}
\begin{proof}
By Theorem \ref{thm:det-property} and Lemma \ref{lem:rand-dense-large-one}, we get an ordered block subsets $L_1,\ldots, L_k$ for $k=O(1)$ such each vertex $u \in L_i$ has at most poly-logarithmic many neighbors in the blocks of $L_1,\ldots, L_j$. We can then orient the edges of the uncolored subgraph obtained by the algorithm of Theorem \ref{thm:det-property}  such that the maximum out-degree is pol-logarithmic. Using the algorithm of Lemma \ref{}, we can complete the coloring by applying the $(deg+1)$ algorithm in $O(\log\log \log n)$ rounds.
\end{proof}
